Isogeometric shape optimization for nonlinear ultrasound focusing

The goal of this work is to improve focusing of high-intensity ultrasound by modifying the geometry of acoustic lenses through shape optimization. The shape optimization problem is formulated by introducing a tracking-type cost functional to match a desired pressure distribution in the focal region. Westervelt's equation, a nonlinear acoustic wave equation, is used to model the pressure field. We apply the optimize first, then discretize approach, where we first rigorously compute the shape derivative of our cost functional. A gradient-based optimization algorithm is then developed within the concept of isogeometric analysis, where the geometry is exactly represented by splines at every gradient step and the same basis is used to approximate the equations. Numerical experiments in a 2D setting illustrate our findings.

==> Lens-Transducer-Picture/Mathematik_Makros.tex <==


                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%                 Mathematik-Makros                  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%  -- N,Z,Q,R,C,...  --  %%%%%%%%%%%%%%%%%%%%%%

	\newcommand{\N}{\mathds{N}}		%(ggf. auf mathbb statt mathds umstellen)
	\newcommand{\Z}{\mathds{Z}}
	\newcommand{\Q}{\mathds{Q}}
	\newcommand{\R}{\mathds{R}}
	\newcommand{\C}{\mathds{C}}
	\newcommand{\K}{\mathds{K}}
	\renewcommand{\H}{\mathds{H}}
	\renewcommand{\O}{\mathds{O}}
	\renewcommand{\S}{\mathbb{S}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






	
%%%%%%%%%%%%%%%%  -- griechische Buchstaben  --  %%%%%%%%%%%%%%%%%

	\renewcommand{\epsilon}{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%  -- Vektoren  --  %%%%%%%%%%%%%%%%%%%%%%%%

	\newcommand{\iivector}[2]{\left( \begin{array}{r}			% 2er-Vektor
										#1 \\
										#2
									 \end{array}\right)}	
		
	\newcommand{\iiivector}[3]{\left( \begin{array}{c}			% 3er-Vektor
										#1 \\
										#2 \\
										#3
									 \end{array}\right)}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%  -- Matrizen  --  %%%%%%%%%%%%%%%%%%%%%%%%

	\newcommand{\iimatrix}[4]{\left( \begin{array}{rr}			% 2x2-Matrix
										#1 & #2 \\
										#3 & #4
									 \end{array}\right)}	
	
	\newcommand{\iiimatrix}[9]{\left( \begin{array}{rrr}		% 3x3-Matrix
										#1 & #2 & #3 \\
										#4 & #5 & #6 \\
										#7 & #8 & #9
									  \end{array}\right)}
		
	\newcommand{\dotmatrix}[6]{\left( \begin{array}{cccc}	    % 4x4-Dot-Matrix
										#1 & #2 & \dots & #3 \\
										#4 & \ddots & & \multirow{2}{*}{\vdots} \\
										\vdots & & \ddots &  \\
										#5 & \multicolumn{2}{c}{\dots} & #6
									  \end{array}\right)}
		
	\newcommand{\dotdet}[6]{\left| \begin{array}{cccc}		% 4x4-Dot-Determinante
										#1 & #2 & \dots & #3 \\
										#4 & \ddots & & \multirow{2}{*}{\vdots} \\
										\vdots & & \ddots &  \\
										#5 & \multicolumn{2}{c}{\dots} & #6
								   \end{array}\right|}
												%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	





							   
%%%%%%%%%%%%%%%%%%%%%%%  -- Symbole  --  %%%%%%%%%%%%%%%%%%%%%%%%%

	\renewcommand{\qed}{\parbox{\textwidth}{\raggedleft $\Box$}}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	






%%%%%%%%%%%%%%%%%%%%  -- Differentiale  --  %%%%%%%%%%%%%%%%%%%%%%

	\newcommand{\dd}{\textup{d}}
	\newcommand{\DD}{\textup{D}}
	\newcommand{\JJ}{\textup{J}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%  -- "Buchstaben-Operatoren"  --  %%%%%%%%%%%%%%%%%

	\newcommand{\tr}{\textup{tr}}
	\newcommand{\intern}{\textup{int }}
	\newcommand{\id}{\textup{id}}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%  -- Hystereseoperatoren  --  %%%%%%%%%%%%%%%%%%%	

	\newcommand{\PP}{\mathcal{P}}
	\newcommand{\WW}{\mathcal{W}}
	\newcommand{\mc}{\psi_{-1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> Lens-Transducer-Picture/Praeambel.tex <==


                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%                      Präambel                      %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%  --  Textsatz  --  %%%%%%%%%%%%%%%%%%%%%%%

\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc}
\usepackage[ngerman]{babel}
\usepackage[babel,german=quotes]{csquotes} % deutsche Anführungszeichen
\usepackage{lmodern}
\parindent 0cm

\usepackage{blindtext}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%  --  Farben  --  %%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{color}

	

%%% MATLAB-Code-Listings %%%
	\definecolor{colKeys}{rgb}{0,0,1}
	\definecolor{colIdentifier}{rgb}{0,0,0}
	\definecolor{colComments}{rgb}{0,1,0.3}
	\definecolor{colString}{rgb}{0,0.5,0}
	\definecolor{dkgreen}{rgb}{0,0.6,0}
	\definecolor{gray}{rgb}{0.5,0.5,0.5}
	\definecolor{lila}{rgb}{0.5,0,0.5}
	
%%% Farben für den Text %%%
	\definecolor{dkred}{rgb}{0.4,0,0}
	\definecolor{dkblue}{rgb}{0,0,0.4}
	\definecolor{ltblue}{rgb}{0,0.5,0.8}
	\definecolor{dlkgreen}{rgb}{0,0.8,0}
	\definecolor{ddkgreen}{rgb}{0,0.4,0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%  --  Seitengestaltung  --  %%%%%%%%%%%%%%%%%%%

\usepackage[top=2cm,bottom=4cm,left=1.5cm,right=1.5cm]{geometry}

\usepackage{scrpage2}
	\cfoot{\pagemark}
	\chead{\headmark}
	\automark{section}
	\setkomafont{pageheadfoot}{\scshape}
	\setkomafont{pagefoot}{\scshape}
	\setkomafont{pagenumber}{\normalfont}
	%\setheadtopline{1pt}[\color{black}]
	\setheadsepline{1pt}[\color{black}]
	%\setlength{\headsep}{50pt}
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%  --  Mathematischer Formelsatz  --  %%%%%%%%%%%%%%%

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{dsfont}								   % \mathds
\usepackage{mathrsfs}							   % \mathscr

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%  --  Bilder/pdfs einbinden  --  %%%%%%%%%%%%%%%%%

\usepackage{graphicx}
\graphicspath{{images/}}
\usepackage{pdfpages}
\usepackage{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%  --  Tabellen  --  %%%%%%%%%%%%%%%%%%%%%%%

\usepackage{threeparttable} 			  %Fußnoten in Tabellen
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{colortbl}
\renewcommand{\arraystretch}{1} 		  % Zeilenhöhe

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%  --  Captions  --  %%%%%%%%%%%%%%%%%%%%%%%%

\addto\captionsngerman{
\renewcommand{\figurename}{Abb.}%
\renewcommand{\tablename}{Tab.}%
					  }
\usepackage{caption}
\renewcommand{\capfont}{\footnotesize}
\renewcommand{\caplabelfont}{\footnotesize\bfseries}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%  --  Referenzierung  --  %%%%%%%%%%%%%%%%%%%%%

\usepackage{nameref}
\usepackage[pdfauthor={Vorname Nachname},pdftitle={Titel},
				colorlinks  = true,
				linkcolor   = blue,
				urlcolor    = blue,
				citecolor   = blue,
				linktoc     = page]
		   {hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%  --  Literaturverzeichnis  --  %%%%%%%%%%%%%%%%%%

\usepackage[printonlyused]{acronym}			    % Abkürzungsverzeichns
\usepackage{bibgerm}						    % "deutscher" Stil für die 														       Bibliothek, erfordert: 														       \bibliographystyle{gerplain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%  --  Theoremstyles  --  %%%%%%%%%%%%%%%%%%%%%%

\newtheoremstyle{theorem}		% name
				{15pt} 			% Space above
				{5pt} 			% Space below 
				{\it} 			% Body font
				{} 				% Indent amount: \parindent = normal paragraph 									  indent
				{\bf} 			% Theorem head font
				{:} 			% Punctuation after theorem head
				{ } 			% Space after theorem head: Space after theorem 								  head: { } = normal interword space;											  \newline = linebreak
				{} 				% Theorem head spec (can be left empty, meaning 								  `normal')



\newtheoremstyle{annotation}	% name
				{15pt} 			% Space above
				{5pt} 			% Space below 
				{} 				% Body font
				{} 				% Indent amount: \parindent = normal paragraph 									  indent
				{\it} 			% Theorem head font
				{:} 			% Punctuation after theorem head
				{ } 			% Space after theorem head: Space after theorem 								  head: { } = normal interword space;											  \newline = linebreak
				{\underline{\thmname{#1}~\thmnumber{#2}}}
				 				% Theorem head spec (can be left empty, meaning 								  `normal')
				 	
				 	
				 				
\newtheoremstyle{defin}			% name
				{15pt} 			% Space above
				{5pt} 			% Space below 
				{} 				% Body font
				{} 				% Indent amount: \parindent = normal paragraph 									  indent
				{\bf} 			% Theorem head font
				{:} 			% Punctuation after theorem head
				{ } 			% Space after theorem head: Space after theorem 								  head: { } = normal interword space;											  \newline = linebreak
				{} 				% Theorem head spec (can be left empty, meaning 								  `normal')

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%  --  Theoreme  --  %%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{theorem}					  % Ab hier alle Theoreme der Klasse 												"theorem"

	\newtheorem{satz}{Satz}[section]	  % Satz als Maintheorem stellt den 												counter
	\newtheorem{lemma}[satz]{Lemma}
	\newtheorem{proposition}[satz]{Proposition}
	\newtheorem{corollar}[satz]{Corollar}



\theoremstyle{annotation}				  % Ab hier alle Theoreme der Klasse 												"annotation"

	\newtheorem{anmerkung}[satz]{Anmerkung}			
	\newtheorem{beispiel}[satz]{Beispiel}



\theoremstyle{defin}					  % Ab hier alle Theoreme der Klasse 												"defin"

	\newtheorem{definition}[satz]{Definition}	
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%  --  MATLAB-Code  --  %%%%%%%%%%%%%%%%%%%%%%%

\usepackage{listings}
\renewcommand\lstlistingname{MATLAB-Code}
\renewcommand\lstlistlistingname{Matlab-Code-Verzeichnis}
\lstset{language=Matlab,
   float=hbp,
   basicstyle=\ttfamily\small,
   identifierstyle=\color{colIdentifier},
   keywordstyle=\color{blue},
   commentstyle=\color{dkgreen},
   stringstyle=\color{lila},
   columns=flexible,
   tabsize=2,
   frame=single,
   numbers=left,
   extendedchars=true,
   showspaces=false,
   numberstyle=\tiny\color{gray},
   stepnumber=1,
   numbersep=10pt,
   showspaces=false,
   showstringspaces=false,
   breakautoindent=true
   keywords={break,case,catch,continue,else,elseif,end,for,function,
   global,if,otherwise,persistent,return,switch,try,while,ones,zeros},
   }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%  --  TikZ  --  %%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}

\usetikzlibrary{intersections}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{positioning}
\usetikzlibrary{petri}
\usetikzlibrary{calc}
\usetikzlibrary{through}
\usetikzlibrary{mindmap}
\usetikzlibrary{trees}
\usetikzlibrary{shadows}
\usetikzlibrary{calendar}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


